Covariant Quantum Gravitational Corrections to Scalar and Tensor Field Models

Recent and upcoming experimental data as well as the possibility of rich phenomenology have spiked interest in studying the quantum effects in cosmology at low (inflation-era) energy scales. One of the approaches to find covariant quantum corrections is the DeWitt-Vilkovisky's (DV) covariant effective action formalism that is gauge invariant and background field invariant. We use the DeWitt-Vilkovisky method to study formal and cosmological aspects of quantum fields in curved spacetime, and take initial steps towards studying quantum gravitational corrections in cosmological setting. The thesis comprises of mainly two parts. We first study the formal aspects of rank-2 antisymmetric tensor field which appear in the low energy limit of superstring models and are thus relevant in the early universe, in particular the quantization and quantum equivalence properties, for the case with and without spontaneous Lorentz violation. The effective action is generalized for gauge theories whose gauge parameters possess additional symmetries. When used in the case of spontaneously Lorentz violating antisymmetric tensor field model, it is found that classical equivalence with a vector theory breaks down at one-loop level due to the presence of Lorentz violating terms. The final chapter of this thesis is devoted to taking first steps towards exploring applications of DV method in early universe cosmology. We calculate perturbatively the covariant one-loop quantum gravitational effective action for a scalar field model inspired by the recently proposed nonminimal natural inflation model. The effective potential is evaluated taking into account the finite corrections, and an order-of-magnitude estimate of the one-loop corrections reveals that gravitational and non-gravitational corrections have same or comparable magnitudes.

==> frontmatter/certificate.tex <==
%!TEX root=../thesis.tex

%\vspace{2cm}
\begin{center}\large{\textbf{CERTIFICATE}}\end{center}
\vspace{0.5cm}
The undersigned have examined the Ph.D. thesis entitled:
\begin{center}\textbf{\thesistitle}\end{center}
presented by \salutation ~\studentname, a candidate for the degree of \mbox{Doctor of Philosophy} in the department of \subject, and hereby certify that it is worthy of acceptance.

\vspace{1cm}
\parbox{0.6\textwidth}{ 
\flushleft{\vivadate\\IISER, Bhopal}
\vspace{16cm}
}
\hfill 
\parbox{0.4\textwidth}{ 
\mbox{\external}\\
External Examiner\\

\vspace{1.3cm}
\mbox{\advisorname}\\
Supervisor\\

\vspace{1.3cm}
\mbox{\memberone}\\
Member\\

\vspace{1.3cm}
\mbox{\membertwo}\\
Member\\

\vspace{1.3cm}
\mbox{\memberthre}\\
Member\\
}

